PnyxDB: a Lightweight Leaderless Democratic Byzantine Fault Tolerant Replicated Datastore

Byzantine-Fault-Tolerant (BFT) systems are rapidly emerging as a viable technology for production-grade systems, notably in closed consortia deployments for nancial and supply-chain applications. Unfortunately, most algorithms proposed so far to coordinate these systems suffer from substantial scalability issues, and lack important features to implement Internet-scale governance mechanisms. In this paper, we observe that many application workloads offer little concurrency, and propose PnyxDB, an eventually-consistent Byzantine Fault Tolerant replicated datastore that exhibits both high scalability and low latency. Our approach is based on conditional endorsements, that allow nodes to specify the set of transactions that must not be committed for the endorsement to be valid. In addition to its high scalability, PnyxDB supports application-level voting, i.e. individual nodes are able to endorse or reject a transaction according to application-defined policies without compromising consistency. We provide a comparison against BFTSMaRt and Tendermint, two competitors with different design aims, and show that our implementation speeds up commit latencies by a factor of 11, remaining below 5 seconds in a worldwide geodistributed deployment of 180 nodes.

==> aws_csv.tex <==
n,min,mean,l25,l50,l75,l95,l99,max,committed_queries
6,85,126,110,134,147,149,150,150,6
30,193,237,209,234,249,300,316,322,30
60,306,445,368,437,511,608,637,640,60
90,568,974,757,982,1173,1305,1364,1383,90
120,969,1760,1393,1866,2086,2321,2389,2413,120
150,1456,2779,2311,2943,3264,3627,3735,3769,150
180,2053,4026,3422,4249,4681,5189,5366,5419,180


==> checkpoints_csv.tex <==
hotspot,time,checkpoints,err
0,3.500029,0.175000,0.123067
0.5,8.000291,0.500000,0.713293
1,1.500010,0.075000,0.111906
1.5,1.500011,0.075000,0.085310
2,5.000049,0.250000,0.226144
2.5,15.500419,0.900000,0.792703
3,7.000055,0.425000,0.288676
3.5,19.000180,1.650000,0.858613
4,28.500226,1.725000,1.732110
4.5,18.100153,1.400000,0.651010
5,10.850445,1.125000,0.680120
5.5,25.700227,1.900000,0.971129
6,11.600134,1.950000,0.799785
6.5,27.900349,2.000000,0.977053
7,54.050439,3.700000,3.053166
7.5,41.052622,4.000000,2.783380
8,24.701000,3.325000,1.161919
8.5,21.250197,2.375000,0.761959
9,18.900192,2.575000,0.828574
9.5,57.850491,4.750000,2.507532
10,68.151390,5.625000,3.575784
10.5,17.101271,3.400000,0.821940
11,20.250424,3.025000,1.134741
11.5,18.150149,3.300000,0.854480
12,15.050141,3.575000,0.779652


==> rollbacks_csv.tex <==
hotspot,rollbacks,err
0,0.000000,0.000000
0.5,0.000000,0.000000
1,0.000000,0.000000
1.5,0.000000,0.000000
2,0.000000,0.000000
2.5,0.000000,0.000000
3,0.000000,0.000000
3.5,0.005124,0.007235
4,0.000000,0.000000
4.5,0.000000,0.000000
5,0.002567,0.005192
5.5,0.002503,0.005062
6,0.010475,0.010180
6.5,0.007611,0.008664
7,0.002593,0.005246
7.5,0.005058,0.007141
8,0.016264,0.012541
8.5,0.002709,0.005479
9,0.005453,0.007699
9.5,0.010794,0.010490
10,0.008284,0.009423
10.5,0.015879,0.012256
11,0.002981,0.005460
11.5,0.005471,0.007724
12,0.011066,0.010754


==> throughput_csv.tex <==
clients,input,bftsmart,tendermint,ours
1,2.000000,1.998083,1.917738,2.009884
2,4.000000,3.661465,3.736387,3.980175
3,6.000000,4.568142,5.447493,5.757334
4,8.000000,5.017230,7.099939,7.791929
5,10.000000,5.305800,8.847906,9.824840
6,12.000000,5.487847,10.035883,11.779928
7,14.000000,5.554517,12.310356,13.033794
8,16.000000,5.616363,13.921940,15.092690
9,18.000000,5.656407,15.312017,16.770717
10,20.000000,5.683365,17.067504,18.624022
11,22.000000,5.694097,17.889424,19.426154
12,24.000000,5.699175,18.671493,20.491077
13,26.000000,nan,20.044417,21.929875
14,28.000000,nan,21.287802,23.247519
15,30.000000,nan,22.430343,24.200837
16,32.000000,nan,21.652640,26.075029
17,34.000000,nan,24.665030,27.106185
18,36.000000,nan,24.931488,26.030589
19,38.000000,nan,25.885580,28.338252
20,40.000000,nan,27.370497,28.910783


==> varying_clients_bftsmart_csv.tex <==
clients,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
1,321,443,383,435,494,566,628,1013,100,341
2,358,3692,2033,3686,5337,6689,6987,7445,200,4119
3,411,11802,6142,11804,17446,22037,22945,23299,300,8471
4,422,21922,11228,21940,32640,41174,42919,43336,400,12337
5,438,32679,16608,32694,48763,61640,64232,64821,500,16106
6,452,43730,22070,43687,65410,82707,86160,86923,600,19777
7,454,55016,27719,55047,82284,104101,108520,109378,700,23195
8,469,66011,33332,66014,98751,124874,130262,131253,800,26427
9,457,77616,38925,77643,116284,146987,153263,154494,900,30016
10,472,88913,44584,88792,133246,168733,175958,177366,1000,33421


==> varying_clients_ours_csv.tex <==
clients,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
1,73,100,88,96,108,140,147,154,100,17
2,66,105,86,98,111,146,160,1524,199,17
3,65,344,88,100,660,756,1257,5085,292,1209
4,63,109,87,99,117,155,179,2687,394,20
5,59,115,84,96,116,149,177,6139,499,19
6,63,121,88,100,117,153,185,5792,598,22
7,60,196,85,97,115,717,1156,14040,688,1139
8,59,125,84,95,113,149,190,12555,792,18
9,60,150,87,99,116,157,874,15671,880,19
10,57,140,84,97,120,161,209,19017,977,21
11,56,145,82,94,113,152,742,20661,1066,20
12,58,195,87,99,117,743,1285,21806,1149,1188
13,57,154,86,97,115,156,211,24334,1249,19
14,59,197,89,102,121,166,1042,26478,1330,23
15,59,298,86,99,118,801,4024,29475,1400,1286
16,62,167,88,102,120,166,1465,25988,1507,24
17,61,185,90,104,126,175,238,30827,1589,26
18,58,227,87,100,121,291,2722,37874,1658,257
19,58,197,86,101,120,166,1390,36970,1775,23
20,60,209,90,103,123,172,1414,38777,1845,30


==> varying_clients_tendermint_csv.tex <==
clients,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
1,661,1152,948,1129,1314,1641,1772,1883,99,317
2,658,1293,986,1184,1442,2275,2854,3073,195,501
3,655,1350,1003,1212,1520,2496,2973,3144,284,581
4,641,1489,1028,1273,1668,3153,3975,4240,372,602
5,670,1551,1062,1329,1714,3246,4134,4379,467,663
6,668,1807,1107,1422,1993,4628,5906,6234,533,824
7,677,1652,1078,1357,1809,3874,4915,5191,653,742
8,665,1630,1083,1376,1770,3782,4821,5139,733,589
9,662,1763,1093,1409,1879,4457,6002,6401,815,541
10,651,1652,1064,1348,1795,3962,5052,5499,907,597
11,678,1873,1125,1475,2078,4659,5824,6155,956,742
12,686,2002,1170,1584,2222,5031,6150,6422,995,623
13,677,2014,1156,1555,2282,5278,6344,6661,1067,774
14,687,1953,1141,1500,2116,5105,6248,6559,1129,507
15,676,1981,1132,1513,2164,5213,6554,6992,1202,579
16,672,2312,1185,1634,2640,6652,7880,8126,1157,790
17,677,2048,1168,1560,2277,5566,6758,7060,1314,822
18,686,2180,1185,1602,2526,6137,7306,7621,1325,1037
19,697,2148,1164,1551,2400,5983,7150,7598,1385,763
20,685,2093,1151,1520,2276,5876,7126,7437,1476,793


==> varying_contention_ours_csv.tex <==
slots,contention_proba,min,mean,l50,l80,l95,l99,max,up,down,committed_queries
500,0.60,64,135,112,149,202,263,516,0,0,1000
200,1.50,64,137,122,153,199,270,6147,0,0,997
100,2.98,58,182,121,159,219,327,11259,0,0,981
50,5.92,72,183,126,156,222,361,10229,0,0,963
30,9.78,59,196,112,139,191,415,13251,0,0,850
25,11.68,61,653,208,522,1152,12939,24931,0,0,389
20,14.50,58,597,187,371,806,14286,25617,0,0,351
10,28.00,59,838,146,378,984,18268,25340,0,0,117


==> varying_hotspot_ours_1s_csv.tex <==
hotspot,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
0,59,103,83,95,112,147,184,1016,500,0
0.5,59,108,85,97,118,155,188,2377,500,0
1,59,104,85,97,115,152,190,840,500,0
1.5,62,107,88,101,119,157,191,294,499,2
2,57,101,81,92,108,145,182,1768,500,0
2.5,62,107,89,101,117,154,191,853,496,6
3,58,104,83,96,113,152,188,1620,500,0
3.5,59,132,87,99,117,154,816,5144,493,8
4,59,109,85,98,113,154,194,2834,499,1
4.5,61,113,87,99,116,157,199,3720,499,1
5,58,107,82,93,110,149,189,2545,497,5
5.5,61,130,88,100,117,155,193,7013,493,5
6,58,115,86,99,116,160,204,4014,496,2
6.5,64,121,91,103,119,158,197,5537,494,4
7,58,120,82,94,111,150,749,4933,495,4
7.5,57,105,82,94,110,148,191,3172,491,6
8,60,115,85,96,111,151,193,5702,494,4
8.5,60,140,87,99,117,157,777,9118,485,6
9,61,112,87,99,117,161,208,3119,489,7
9.5,58,117,84,97,117,155,190,6339,487,6
10,57,122,83,95,111,148,189,8727,485,7
10.5,59,141,83,95,112,655,800,4873,483,9
11,63,130,91,103,120,158,199,8670,483,6
11.5,56,113,80,91,109,151,198,6026,478,8
12,57,125,84,96,117,154,768,5380,474,8


==> varying_hotspot_ours_2s_csv.tex <==
hotspot,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
0,62,118,94,110,133,180,234,900,250,0
1,65,120,95,110,133,184,243,1780,250,0
2,65,129,101,119,144,195,252,3118,249,2
3,68,115,95,108,126,169,215,832,250,0
4,66,113,92,103,119,159,204,3504,249,1
5,69,116,95,108,127,170,219,963,250,0
6,63,111,88,100,119,158,205,1512,248,2
7,68,121,94,106,125,167,246,2270,249,1
8,69,127,94,108,126,168,331,3140,247,2
9,63,119,88,101,119,161,281,2998,248,1
10,67,134,93,105,125,171,760,3403,247,2
11,63,131,90,103,121,164,295,4434,244,3
12,71,128,97,109,129,173,330,2204,247,2
13,64,134,88,101,119,161,463,4578,243,4
14,67,140,93,105,123,170,324,7185,237,6
15,65,139,91,104,120,162,270,5704,239,4
16,67,161,94,107,126,169,804,7496,236,5
17,66,138,92,104,123,169,788,4464,239,5
18,67,152,93,106,124,169,607,6908,228,7
19,66,142,92,105,122,163,312,5305,227,7
20,67,146,92,105,123,170,343,5858,226,7


==> varying_hotspot_ours_applied_csv.tex <==
hotspot,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
0,61,104,87,98,112,148,184,1458,1000,0
0.5,60,108,88,101,118,153,187,2101,999,1
1,56,101,82,94,112,149,190,627,1000,0
1.5,57,102,83,94,113,158,197,573,995,9
2,59,103,84,95,112,151,190,1684,999,0
2.5,57,103,83,96,111,148,183,2299,997,2
3,59,105,85,98,113,150,190,1636,998,1
3.5,60,106,86,98,115,154,193,1695,991,7
4,58,104,85,97,113,152,191,1186,990,7
4.5,61,109,87,100,116,159,199,2346,988,5
5,60,106,87,98,114,153,193,1407,988,11
5.5,57,102,81,93,109,147,186,2549,984,7
6,56,103,84,96,112,149,186,1355,975,12
6.5,61,108,88,100,116,153,188,2488,972,16
7,56,103,82,94,111,147,294,1295,972,16
7.5,57,111,84,99,117,153,339,3540,962,16
8,58,103,84,96,113,151,191,1791,958,12
8.5,59,105,84,96,113,154,195,1815,963,9
9,60,106,86,97,113,153,193,2756,941,15
9.5,60,107,85,97,113,151,278,2392,933,15
10,58,109,84,96,116,155,391,2706,930,20
10.5,59,104,84,96,112,149,191,2507,936,14
11,61,108,88,101,118,156,196,2260,923,19
11.5,59,106,86,98,116,156,199,1216,925,13
12,61,107,87,99,116,156,196,1248,915,12


==> varying_hotspot_ours_csv.tex <==
hotspot,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
0,61,108,87,98,112,148,184,5197,1000,0
0.5,60,111,88,101,118,153,187,4762,999,1
1,56,103,82,94,112,149,190,1712,1000,0
1.5,57,104,83,94,113,158,197,2193,995,9
2,59,107,84,95,112,151,190,5419,999,0
2.5,57,108,83,96,111,148,183,6525,997,2
3,59,110,85,98,114,150,190,5982,998,1
3.5,60,111,86,98,115,154,193,6562,991,7
4,58,128,85,97,113,152,746,5559,990,7
4.5,61,119,87,100,116,159,199,9841,988,5
5,60,110,87,98,114,153,193,5700,988,11
5.5,57,109,81,93,109,147,186,7376,984,7
6,56,107,84,96,112,149,186,5659,975,12
6.5,61,114,88,100,116,153,188,7687,972,16
7,56,172,82,94,111,674,1478,7110,972,16
7.5,57,162,84,99,117,703,899,8525,962,16
8,58,107,84,96,113,151,191,5159,958,12
8.5,59,112,84,96,113,154,195,7874,963,9
9,60,113,86,97,113,153,193,9172,941,15
9.5,60,157,85,97,113,676,825,12551,933,15
10,58,194,84,96,116,1224,1526,9681,930,20
10.5,59,108,84,96,112,149,191,5273,936,14
11,61,114,88,101,118,156,196,7683,923,19
11.5,59,110,86,98,116,156,199,3928,925,13
12,61,112,87,99,116,156,196,5652,915,12


==> varying_n_bftsmart_csv.tex <==
n,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
10,452,469,458,464,474,495,504,506,1,50
20,619,666,627,635,682,769,821,834,2,86
40,1946,2414,2085,2262,2584,3336,3835,4007,4,231


==> varying_n_ours_csv.tex <==
nodes,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
10,85,105,94,102,112,133,141,143,1,16
20,76,102,83,90,105,155,200,212,2,15
40,81,115,89,99,119,197,269,292,4,11
80,99,137,111,123,143,222,296,350,8,11
160,231,424,374,438,484,517,531,544,15,6
320,960,1735,1475,1655,1776,2215,5131,10896,30,484


==> varying_n_tendermint_csv.tex <==
nodes,min,mean,l25,l50,l75,l95,l99,max,committed_queries,err
10,992,1046,1023,1040,1066,1102,1114,1117,1,64
20,1320,1386,1362,1383,1408,1440,1460,1465,2,95
40,1290,1336,1317,1333,1350,1382,1409,1419,4,112
80,2185,2305,2255,2300,2347,2419,2470,2510,8,152
160,11600,13303,12086,12971,14142,16033,17356,18583,16,1014

